Pose Estimation for Objects with Rotational Symmetry

Pose estimation is a widely explored problem, enabling many robotic tasks such as grasping and manipulation. In this paper, we tackle the problem of pose estimation for objects that exhibit rotational symmetry, which are common in man-made and industrial environments. In particular, our aim is to infer poses for objects not seen at training time, but for which their 3D CAD models are available at test time. Previous work has tackled this problem by learning to compare captured views of real objects with the rendered views of their 3D CAD models, by embedding them in a joint latent space using neural networks. We show that sidestepping the issue of symmetry in this scenario during training leads to poor performance at test time. We propose a model that reasons about rotational symmetry during training by having access to only a small set of symmetry-labeled objects, whereby exploiting a large collection of unlabeled CAD models. We demonstrate that our approach significantly outperforms a naively trained neural network on a new pose dataset containing images of tools and hardware.

==> results_orig_table.tex <==
\vspace{-1mm}
\section{Experimental Results}
\label{sec:results}
\vspace{-1mm}


In this section we evaluate our method. We report our performance on the real dataset, and ablate the use of the CAD model collection and the synthetic dataset.  We evaluate with both discretization schemes ($ N = 80 $ and $ N = 168 $ viewpoints). We first describe our evaluation metrics in~\secref{sec:eval_metric} and show quantitative and qualitative results in~\secref{sec:res_quant} and~\secref{sec:res_qual} respectively.

\begin{table}[t!]
\vspace{-0mm}
	\centering
	\setlength{\tabcolsep}{2.8pt}
	\begin{tabular}{|c||c|c|c||c|c|c|}
		\hline
		Using  & \multicolumn{3}{c||}{$ N = 80 $ } & \multicolumn{3}{c|}{$ N = 168 $} \\
		\cline{2-7} 
		 constraints  & { Recall }      & { Prec.}       & {F1 }     & {Recall}       & {Prec.}       & { F1  }     \\
		\hhline{|=#=|=|=#=|=|=|}
		%\multicolumn{1}{|l|}{Handcrafted method}                                                                                                                                                              &              &                 &         &              &                 &          \\ \hline
		%\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Binary CE Loss on match/not-match, \\ fixed conversion from ranking to match/not-match\end{tabular}}                                                  &              &                 &         &              &                 &          \\ \hline
		%\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}Binary CE Loss on match/not-match, \\ fixed conversion from ranking to match/not-match,\\ considering theoretical limits\end{tabular}}                &              &                 &         &              &                 &          \\ \hline
		\ding{55}                      &    97.4       &      96.3        &   0.968     &    91.2     &      90.6           &    0.909          \\ \hline
		\ding{51} &      100.0       &         100.0      &    1    &     96.3     &        97.6       &    0.967     \\ 
		\hhline{|=#=|=|=#=|=|=|}
		 Baselines &     \multicolumn{2}{c|}{Recall}      &     \multicolumn{2}{c|}{Prec.}        &   \multicolumn{2}{c|}{F1}   \\ \hline
		 Baseline ICP &     \multicolumn{2}{c|}{77.8}      &     \multicolumn{2}{c|}{91.7}        &   \multicolumn{2}{c|}{84.2}     \\ \hline
		 Baseline paper &    \multicolumn{2}{c|}{58.3}      &     \multicolumn{2}{c|}{68.2}        &   \multicolumn{2}{c|}{62.9}     \\ \hline
		\end{tabular} 
		\vspace{0.4mm}
			\caption{{\bf Rotational Symmetry Performance.} For different choices of discretization, $ \bf N $, we report \textit{recall}, \textit{precision} and \textit{F1} measures, averaged across the $4$ symmetry classes. Numbers are in \% . {\color{magenta} Missing proper format + running times of each}}
		%\caption{ {\color{red} Same table but results measured differently. Here, recall and prec where measured by doing mean of recall and precision of each class. In the other one, recall by summing all true positives dividing by all false positives, independently of the class. And similarly for precision. Which table? Similar results} }
		\label{tab:results_sym}
		\vspace{-2mm}
\end{table} 

\vspace{-1mm}
\subsection{Evaluation Metrics} 
\label{sec:eval_metric} 

\paragraph{Rotational Symmetry Classification} For rotational symmetry classification, we report the mean of \textit{precision}, \textit{recall} and the \textit{F1} scores of the order predictions across different rotational axes ($ \bX, \bY, \bZ $) and object models.

%\vspace{-3mm}
\paragraph{Pose Estimation} For pose estimation, we report the recall performance (R@$ d_\text{rot}^{sym} $) for our top-k predictions. Using the distance measure in the quaternion space, $ d_\text{rot}^{sym} $ (defined in~\secref{sec:loss_func}), we compute the minimum distance of the ground truth pose wrt our top-k predictions and report how many times this distance falls below $ 20^{\circ} $ or $ 40^{\circ} $. The choice of these values are based on the fact that the distance between two adjacent viewpoints for $ N = 80 $ and $ N = 168 $ discretization schemes are $ 21.2^\circ $ and $ 17.8^\circ $, respectively. We also report the average spherical distance, $ d_\text{rot, avg}^{sym} $ of the best match among the top-k predictions relative to the ground truth pose. In all our experiments, we choose top-5\% of the total possible viewpoints, \ie, for $ N = 80 $ and $ 160 $ discretization schemes, $k = 4$ and $8$, respectively.

\begin{figure*}[t!]
\vspace{-3mm}
\begin{minipage}{0.52\linewidth}
	\centering
	\setlength{\tabcolsep}{-5pt}
	\begin{tabular}{cc}
		 \includegraphics[trim={0 0 50 0}, clip = true,width=0.5\linewidth]{figs/res_timestamp_80} & \includegraphics[trim={0 0 50 0}, clip = true,width=0.5\linewidth]{figs/res_1034_80} \\
		 (a) \textit{Timestamp}-based split & (b) \textit{Object}-based split
		%		\includegraphics[trim={0 0 0 0}, clip = true,width=8cm]{figs/res_timestamp_168.png} \\
		%		\includegraphics[trim={0 0 0 0}, clip = true,width=8cm]{figs/res_1034_168.png}
	\end{tabular} 
	\vspace{0.5mm}
	\caption{{\bf Recall vs spherical distance}}
	\label{fig:pose_plots}
	\end{minipage}
	\hspace{-1mm}
	\setlength{\tabcolsep}{-0pt}
	\begin{minipage}{0.485\linewidth}
		\begin{tabular}{cc}
%		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/image0.png}   \\
 		\includegraphics[trim={3cm 2.0cm 1.5cm 2.4cm}, clip = true,width=0.5\linewidth]{figs/image1.png}  &
%		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/image2.png}  \\
%		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/image3.png}  \\
		\includegraphics[trim={3cm 2.0cm 1.5cm 2.4cm}, clip = true,width=0.5\linewidth]{figs/image4.png}  \\
%		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/image5.png}  \\
%		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/image6.png}  \\
%		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/image7.png}  \\
		\includegraphics[trim={3cm 2.0cm 1.5cm 2.0cm}, clip = true,width=0.5\linewidth]{figs/image8.png}  &
		\includegraphics[trim={3cm 2.0cm 1.5cm 2.4cm}, clip = true,width=0.5\linewidth]{figs/image9.png}
	\end{tabular}
	\centering
	\caption{Qualitative results for pose estimation. Green box indicates correct viewpoint. The bottom-right  shows an error case. }
	\label{fig:epson1034_result}
	\end{minipage}
		\vspace{-3mm}
\end{figure*}


\begin{figure}[t!]%[!htbp]
\vspace{-4mm}
	\centering
	\resizebox{1.06\linewidth}{!}{
	\setlength{\tabcolsep}{1pt}
	\begin{tabular}{ccc}
		\hspace{-0.25cm}\includegraphics[trim={0 0 0cm 0}, clip = true,width=3.3cm]{figs/obj1.pdf} & 
		\hspace{-0.15cm}\includegraphics[trim={0cm 0 0 0}, clip = true,width=3.3cm]{figs/obj2.pdf} &
		\hspace{-0.15cm}\includegraphics[trim={0 0 0 0}, clip = true,width=3.3cm]{figs/obj3.pdf} \\
		\hspace{-0.25cm}{\scriptsize $X \sim 1, Y \sim 1, Z \sim \infty.$ } & \hspace{-0.5cm}{\scriptsize $X \sim 1, Y \sim 2, Z \sim 1.$} & \hspace{-1cm}{\scriptsize $X \sim 2, Y \sim 1, Z \sim 1.$} \\
		\hspace{-0.25cm}\includegraphics[trim={0 0 0 0}, clip = true,width=3.3cm]{figs/obj4.pdf} &
		\hspace{-0.15cm}\includegraphics[trim={0 0 0 0}, clip = true,width=3.3cm]{figs/obj5.pdf} & 
		\hspace{-0.15cm}\includegraphics[trim={0 0 0 0}, clip = true,width=3.3cm]{figs/obj6.pdf} \\
		\hspace{-0.25cm}{\scriptsize $X \sim 2, Y \sim 2, Z \sim \infty.$} & \hspace{-0.5cm} {\scriptsize $X \sim 1, Y \sim 2, Z \sim 1.$} & \hspace{-1cm}{\scriptsize $X \sim 2, Y \sim 2, Z \sim 2.$ }
	\end{tabular}
	}
	\vspace{-2mm}
	\caption{Examples of our predicted symmetry. The variability of rotational symmetry shows in bottom-left and bottom-right objects. Notice that these objects have higher order of symmetry (eg 6 and 8) than what we consider, for which our model predicts $\mathcal{O}_\infty$. }
	\label{fig:symmetries_inferred}
	\vspace{-2mm}
\end{figure}

\subsection{Quantitative Results} 
\label{sec:res_quant} 


\paragraph{Rotational Symmetry Prediction} We have rotational symmetry annotations for all 17 objects in the real dataset and 28 objects in the synthetic dataset. We split these into 25 objects for training, 10 for validation, and 10 for test. 

% In this case we are interested in increasing the recall. Since the inferred symmetries are being used to train the pose estimation model in a structured ranking loss, assuming a higher level of symmetry for an object implies the network is not learning as much from it. However, ignoring symmetries implies imposing a margin on the Hinge Loss for views that are actually correct.

We show our quantitative results in~\tabref{tab:results_sym}. The first row shows the performance of our approach by considering order prediction for multiple axes to be independent. In the second row, we show that by reasoning about impossible order configurations,  the performance of our symmetry prediction improves. At a finer discretization, we are also able to predict $\mathcal{O}_3$, making the difference even more evident.

{\color{magenta} We compare our method to two baselines. First, we use one iteration of ICP to match the shape of a CAD model to itself having rotated $180^{\circ}$, $90^{\circ}$ and $45^{\circ}$, to detect orders 2, 4 and $\infty$ respectively. When the matching error is smaller than a threshold tuned on the training data, we predict the corresponding order is true. This process is done for each of the three axes considered independently.

The second method \cite{Symmetry17} finds equivalent points in the mesh. We obtain the amount of these points that are explained by every rotational order considered and, based on a threshold tuned on the train data, we predict order of symmetry in each axis. This baseline works well when the object considered has only one axis with symmetry, but fails to explain symmetries in more than one axis.}

% \multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}End-to-end + CE loss on MLP + learnt sigmoid conversion\\ + trained on 6000 objs ignoring symmetry \\ + theoretical limits at inference\end{tabular}} 

%\vspace{-3mm}
\paragraph{Pose Estimation}~\tabref{tab:results_pose} reports results for pose estimation for different configurations. The first column corresponds to the the choice of the dataset split, \textit{timestamp}-based  or \textit{object}-based. The second column indicates the usage of the large-scale synthetic objects while training our network. In the third column, we indicate whether the symmetry prediction was used for the synthetic objects during training. The fourth column indicates whether the symmetry annotations from the real dataset was used as a supervisory signal to adjust our training loss. For each discretization scheme, we report results for R@$  d_\text{rot}^{sym} $ ($ \phi \in  \{ 20^{\circ}, 40^{\circ} \} $) and $ d_\text{rot, avg}^{sym} $ metrics.

We first notice that a model that uses symmetry labels in our loss function, significantly improves the results (first and second row for each dataset split) over the naively trained network. This showcases that reasoning about symmetry is important. Furthermore,  exploiting the additional large synthetic dataset outperforms the base model which only sees the real imagery (first and third rows). Finally, our full model that jointly reasons about symmetry and pose significantly outperforms the rest of the settings. 
%Furthermore, symmetry plays an important role. 
%Furthermore, we show how these factors become more prominent when we want to generalize to unseen objects.  

%The first row corresponds to the baseline approach, \ie, only using the small-sized real dataset without reasoning about rotational symmetry. We can see how using the symmetry labels for just the small set of real images (second row) can improve the quality of embeddings to disambiguate rotational symmetries(third row). While adding a large amount of data can help the network to train better (third row), this improvement is orthogonal to reasoning about rotational symmetries (fourth row). Thus we can see that the accuracy is improved by more than 1.5x when the predicted symmetry labels of the synthetic dataset can be used to scale rotational symmetries to large data. Thus we can see how inferring the symmetries on a large dataset of 3D CAD models and utilize them to train a better embedding function for pose matching. We can also see that using a finer discretization can help us achieve better results at the cost of more computations. 

In~\figref{fig:pose_plots}(a) and (b), we plot  recall vs the spherical distance between the predicted viewpoint and the GT viewpoint for $ N = 80 $ discretization scheme. Since the objects are shared across the splits in the timestamp based data, the overall results are better than the corresponding numbers of the object-based split. However, the improvement of using large-scale synthetic data and rotational symmetries has a roughly 1.7x improvement for object-based split compared to around 1.4x improvement for the timestamp-based split. This shows that for generalization, reasoning about rotational symmetry on a large dataset is essential.  


% For the timestamp based split, we can see how using the symmetry labels for even small-scale datasets (second row) during our training step can improve the pose estimation results. Even without using the symmetry labels, using the large scale synthetic dataset (third row) can improve the performance significantly. The fourth row shows that using both a large scale dataset and just the small-scale symmetry labels can boost performance by {\color{red} xx\%}. However the best performance comes when we use supervision from both the predicted symmetry labels of the synthetic dataset along with the annotated symmetry labels of the real dataset. {\color{red} not true for 168 views.} 

Only using the synthetic objects (green plot) can be better than using the symmetry labels for the small real dataset (red and brown plots). However, combining rotational symmetries with large-scale synthetic data (blue plot) gives the best performance. %This shows that both large-scale datasets and reasoning about symmetry are essential for generalizing the pose estimation performance for unseen objects.
 Please refer to the supplementary material
\footnote{{\color{magenta} Available at \url{www.cs.utoronto.ca/~ecorona/supplementary_rotationalsymm.pdf}} }
 for the $ N = 160 $ discretization scheme as well.

% Having trained on the large synthetic database, the network achieves its maximum performance in a few iterations of fine-tuning on the real data. In this process, the network can take advantage of seeing objects of relatively similar complexity in the simulated environment. 

%{\color{red} compare timestamp based split and object split}% For timestamp based split, 

% For 168 views, the networks need much more time to train since a whole training step needs to forward and back propagate to all the views. The networks need around half a day to converge, whereas, for 80 views, a few hours is enough. For this reason, the hyperparameters of the network where tuned for the 80 views case, extrapolating to when having more views.

%We notice that for the time split symmetry handling has a big effect in improving the results. In this case there is no need to scale to new objects, so the effect of using symmetries is more important than being pretrained on a bigger amount of data. The model learns well the shape of the CAD models to be able to generalize in the test set.

% Differently, when tested on different types of objects, it shows useful to have been trained on an extensive set of synthetic objects. When the model is not trained with symmetries, it can learn to maximize the similarity score of similar images even though the labels can be noisy. 

% In general, synthetic data is significantly more challenging than the real data, having hard lighting conditions, occlusions and a very varying viewpoint position. When the model is refined in the real data, the CNN encoding the scene has to learn the differences. In this case, we  there is an important overfitting to the real scenes, formed by a small set of different objects.

% We also show the $ R@\phi $ vs $ \phi $ plot in~\figref{fig:pose_plots} for $ N = 80 $ discretization scheme.  Please refer to the supplementary material for additional plots for the $ N = 168 $ discretization scheme.


\subsection{Qualitative Results}
\label{sec:res_qual} 

We show the qualitative results of our method in both real and synthetic data.

%\vspace{-4mm}
\paragraph{Symmetry Prediction} We qualitatively observe how our symmetry prediction generalizes to unseen objects at test time. One of the primary reasons for failure is the non-alignment of viewpoints due the discretization. %Since circular shapes (having infinite order of symmetry) can only be represented by a discrete set of vertices, which if not aligned with the coarse viewpoints can result in failure to detect infinite order rotational symmetry. 
Another reason of failure is that examples of certain order classes are not present in training. For example, the object in the bottom left of~\figref{fig:symmetries_inferred}) has an order eight symmetry which was not present in the training set. 


%Cases of failure can be mostly because of subtly differences in the shape of the network that do not weigh enough to the network to break symmetries. When predicting symmetry from a projected mesh, we lose information and some views can look perfectly symmetric because other symmetry-breaking parts are occluded.


\iffalse
\begin{figure}%[!htbp]
	\centering
	\begin{tabular}{cc}
		\includegraphics[trim={0 0 0 0}, clip = true,width=4cm]{figs/obj1.pdf} & 
		\includegraphics[trim={0 0 0 0}, clip = true,width=4cm]{figs/obj2.pdf} \\
		$X \sim 1, Y \sim 1, Z \sim \infty.$ & $X \sim 1, Y \sim 2, Z \sim 1.$ \\
		\includegraphics[trim={0 0 0 0}, clip = true,width=4cm]{figs/obj3.pdf} &
		\includegraphics[trim={0 0 0 0}, clip = true,width=4cm]{figs/obj4.pdf} \\
		$X \sim 2, Y \sim 1, Z \sim 1.$ & $X \sim 2, Y \sim 2, Z \sim \infty.$ \\
		\includegraphics[trim={0 0 0 0}, clip = true,width=4cm]{figs/obj5.pdf} & 
		\includegraphics[trim={0 0 0 0}, clip = true,width=4cm]{figs/obj6.pdf} \\
		$X \sim 1, Y \sim 2, Z \sim 1.$ & $X \sim 2, Y \sim 2, Z \sim 2.$ 
	\end{tabular}
	\caption{Sample models among the 6669 unlabelled objects. We test our method to predict symmetry on new objects to infer their symmetry. Yellow, black and blue stand for X, Y and Z axes respectively. As seen in the last example, which should be $X \sim 2, Y \sim 2, Z \sim 6.$, some special orders cannot be directly captured with our initial discretized views. }
	\label{fig:symmetries_inferred}
\end{figure}
\fi

%\vspace{-4mm}
\paragraph{Pose Estimation} We show qualitative results in~\figref{fig:epson1034_result}. In particular, we show images of objects from the real dataset in the first column, followed by the top-3 viewpoint predictions. The views indicated with a green box correspond to the ground truth. 
Most of the errors are due to the coarse discretization. If the actual pose lies in between two neighboring viewpoints, some discriminative parts may not be visible from either of the coarse viewpoints. This can lead to confusion of the matching network.

% We observe several typical difficulties in pose estimation solutions. First, the simulated images have a large range of illumination conditions. Some mistakes are caused by hard illumination conditions where it is significantly more difficult to understand images.

% Although we do not directly create occlusions, objects can be also occluded in the synthetic scenes in oblique viewpoints, as in the example of the first row. It is also common that the cropped image of the object in the scene does not only contain the object of interest, but also information about the rest of the scene which may include other objects. 



%Finally, in both synthetic and real data, m

\iffalse
\begin{figure}[t!]
	\begin{tabular}{c}
%		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/image0.png}   \\
 		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.4cm}, clip = true,width=8cm]{figs/image1.png}   \\
%		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/image2.png}  \\
%		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/image3.png}  \\
		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.4cm}, clip = true,width=8cm]{figs/image4.png}  \\
%		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/image5.png}  \\
%		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/image6.png}  \\
%		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/image7.png}  \\
%		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/image8.png}  \\
		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.4cm}, clip = true,width=8cm]{figs/image9.png}
	\end{tabular}
	\centering
	\caption{Qualitative results for pose estimation in the real images. A box indicates in green below each view if it is the nearest to the scene on the left. The last row shows an error case, where the pose of the object lies further to its nearest views. }
	\label{fig:epson1034_result}
\end{figure}
\fi





\iffalse
\begin{figure}[t!]
	\begin{tabular}{c}
		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/6000objs1.png}  \\
		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true, width=8cm]{figs/6000objs2.png} \\
		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/6000objs3.png} \\
		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/6000objs4.png} \\
		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/6000objs5.png} \\
		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/6000objs6.png} \\
		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/6000objs8.png} \\
		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/6000objs10.png} \\
		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/6000objs9.png} \\
		\includegraphics[trim={1.0cm 2.0cm 1.0cm 2.0cm}, clip = true,width=8cm]{figs/6000objs7.png}
	\end{tabular}
	\centering
	\caption{Many qualitative results to choose from, using the 6000 objects. This is a sample from the validation set. Two last rows are mistakes (Pose estimation, mistake on ground truth because of symmetry prediction) }
	\label{fig:6000objs_result}
\end{figure}
\fi



==> rotational_order2.tex <==
\section{Our Approach}
\label{sec:method}

We tackle the problem of pose estimation in the presence of rotational symmetry. In particular, we assume we are given a test RGB image of an object unseen at training time, as well as the object's 3D CAD model. Our goal is to compute the pose of the object in the image by matching it to the rendered views of the CAD model. To be robust to mismatches in appearance between the real image and the textureless CAD model, we exploit rendered depth maps instead of RGB views. 
Fig.~\ref{fig:problem} visualizes an example image of an object, the corresponding 3D model, and rendered views. 

\begin{figure}[t!]
\scalebox{0.65}[0.65]{
\addtolength{\tabcolsep}{-4.5pt}
	\begin{tabular}{cccccc}
		\includegraphics[trim={0 0 0 0}, clip = true,width=2cm]{figs/object_scene.png}  &
		\includegraphics[trim={14cm 6.5cm 13cm 6cm}, clip = true, width=2cm]{figs/CAD_view.jpg} &
		\includegraphics[trim={3.5cm  1.5cm 3.5cm 1.5cm }, clip = true,width=2cm]{figs/view1.png}&
		\includegraphics[trim={3.5cm  1.5cm 3.5cm 1.5cm }, clip = true,width=2cm]{figs/view2.png} &
		\includegraphics[trim={3.5cm  1.5cm 3.5cm 1.5cm }, clip = true,width=2cm]{figs/view3.png} &
		\includegraphics[trim={3.5cm  1.5cm 3.5cm 1.5cm }, clip = true,width=2cm]{figs/view_correct.png} \\
		(image) & (CAD model) & \multicolumn{4}{c}{(rendered CAD views (depth maps))}\\
	\end{tabular}
	}
	\centering
	\vspace{0.1mm}
	\caption{\small Our problem entails estimating the pose of the object in the image (left) given its CAD model. We exploit rendered depth images of the CAD model in order to determine the pose.}
	\label{fig:problem}
	\vspace{-1mm}
\end{figure}

Our approach follows~\cite{wohlhart2015learning} in learning  a neural network that embeds a real image and a synthetic view in the joint semantic space. In order to perform pose estimation, we then find the view closest to the image in this embedding space. As typical in such scenarios, neural networks are trained with e.g. a triplet loss, which aims to embed the matching views closer than any of the non-matching views. However, in order for this loss function to work well, ambiguity with respect to rotational symmetry needs to be resolved. That is, due to equivalence of shape under certain 3D rotations for rotationally symmetric objects, certain rendered viewpoints look exactly the same. If such  views are used as negative examples during training, we may introduce an ambiguity that prevents us in learning a better model. Note that this is not true for other symmetries such as a reflective symmetry, since the object does not necessarily have equivalent shape in different 3D poses. 
 We propose to deal with this issue by inferring reflectional symmetries of objects, and exploiting them in designing a more robust loss function. 

We first provide basic concepts of rotational symmetry in~\secref{sec:rot_sym}. In Sec.~\ref{sec:method}, we propose our neural network for joint pose and symmetry estimation, and introduce a loss function that takes into account equivalence of certain views. %In Subsec.~\ref{sec:rot_infer}, we propose a network that infers orders of symmetry for an object using only a small number of training examples. 
We show how to train this network by requiring only a small set of symmetry-labeled objects, and by exploiting a large collection of unlabeled CAD models crawled from the web. 


\subsection{Rotational Symmetry}
\label{sec:rot_sym}


We start by introducing notation and basic concepts. 

%\vspace{-4mm}
\paragraph{Rotation Matrix} We denote a rotation of an angle $\phi $ around an axis $ \theta $ using a matrix $ \mathbf{R}_{\theta} (\phi) $. For example, if the axis of rotation is the X-axis, then

\[
\mathbf{R}_{X} (\phi) = \left[ \begin{array}{ccc}
1 & 0 & 0 \\
0 & \cos{\phi} & - \sin{\phi}   \\
0 & \sin{\phi}  & \cos{\phi}  \\
\end{array} \right]
\]

\paragraph{Order of Rotational Symmetry} We say that an object  has an $n$  order of rotational symmetry around the axis $ \theta $, \ie, $ \mathcal{O}(\theta) = n $, when its 3D shape is equivalent to its shape rotated by $ \mathbf{R}_{\theta} \left( \dfrac{2 \pi i}{n} \right), \forall i \in \{0, \ldots, n - 1\} $. % Thus, $ \mathcal{O}_{\theta} (x) = \mathcal{O}_{\theta} (x) =  $


The min value of $ \mathcal{O}(\theta) $ is 1, and holds for objects non-symmetric around axis $\theta$. The max value is $ \infty $, which indicates that the 3D shape is equivalent when rotated by any angle around its axis of symmetry. This symmetry is also referred to as the revolution symmetry~\cite{bregier2017symmetry}. In ~\figref{fig:rot_sym}, we can see an example of our rotational order definition. For a 3D model shown in~\figref{fig:rot_sym} (a), the rotational order about the $ \bY $ axis is 2, \ie, $ \mathcal{O} (\bY) = 2 $. Thus for any viewpoint $ v $ (cyan) in~\figref{fig:rot_sym} (b), if we rotate it by $ \pi $ about the Y-axis to form, $ v_\pi = \mathbf{R}_{\bY} (\pi) v $, the 3D shapes will be equivalent (\figref{fig:rot_sym} (right)). The 3D shape in any other viewpoint (such as, $ v_{\pi/4} $ or $ v_{\pi/2} $) will not be equivalent to that of $ \bv $. Similarly, we have $ \mathcal{O} (\bZ) = \infty $. 
In our paper, we only consider the values of rotational order to be one of $ \{ 1, 2, 4, \infty \} $, however, our method will not depend on this choice. 


\begin{figure}[t!]
	\scalebox{0.5}[0.5]{
		\begin{tabular}{ccc}
			\raisebox{0.2\height}{\includegraphics[trim={0 0 0 0}, clip = true,width=3.6cm]{figs/rot_sym1.jpg}}
			\put(-110,44){\Large $ \bX $} 
			\put(-9,50){\Large  $ \bY $}
			\put(-62,149){\Large $ \bZ $} & 
			\includegraphics[trim={0 0 0 0}, clip = true,width=5.9cm]{figs/rot_sym2.jpg}
			\put(-12, 60){\Large $ \bX $}
			\put(-105, 155){\Large $ \bZ $}
			\put(-64, 84){\Large $ \theta $}
			\put(-33, 128){\LARGE $ v $}
			\put(-160, 10){\LARGE $ v_\pi $}
			\put(-124, 88){\huge $ \pi $} &
			\includegraphics[trim={0 0 0 0}, clip = true,width=5.9cm]{figs/rot_sym_v2.jpg}  \\
			{\LARGE (a) 3D Model} & {\LARGE (b) XZ plane}  
		\end{tabular}
	}
	\vspace{1mm}
	\caption{Order of Rotational Symmetry. An object has $n$th order of rotational symmetry over an axis when its 3D shape is equivalent when rotated $ \left( \dfrac{2 \pi i}{n} \right), \forall i \in \{0, \ldots, n - 1\} $ over this axis. For example, the cylinder in (a) has rotational symmetry over the axes X, Y and Z. In (b), we show its second order of symmetry over the axis Y, as the shape repeats every $\pi$.}
	\label{fig:rot_sym}
\end{figure}


\iffalse
\begin{figure}[t!]
\scalebox{0.5}[0.5]{
	\begin{tabular}{cc}
		\hspace{-0.0cm}
		\raisebox{0.2\height}{\includegraphics[trim={0 0 0 0}, clip = true,width=3.6cm]{figs/rot_sym1.jpg}}
		\put(-110,44){\Large $ \bX $} 
		\put(-9,50){\Large  $ \bY $}
		\put(-62,149){\Large $ \bZ $} & \hspace{-.0cm}
		\includegraphics[trim={0 0 0 0}, clip = true,width=5.9cm]{figs/rot_sym2.jpg}
		\put(-12, 60){\Large $ \bX $}
		\put(-105, 155){\Large $ \bZ $}
		\put(-64, 84){\Large $ \theta $}
		\put(-33, 128){\LARGE $ v $}
		\put(-160, 10){\LARGE $ v_\pi $}
		\put(-124, 88){\huge $ \pi $} \\
		{\LARGE (a) 3D Model} & {\LARGE (b) XZ plane} 
	\end{tabular}} \hspace{-.2cm}
	 \begin{tabular}{cc}%[c]{@{}l@{}}   
	\includegraphics[trim={10cm 2cm 10cm 2cm}, clip = true,width=1.2cm]{figs/view0.png} & \hspace{-0.5cm}
	\includegraphics[trim={10cm 2cm 10cm 2cm}, clip = true,width=1.2cm]{figs/view180.png} \\
	$ v $ & \hspace{-0.5cm} $ v_\pi $ \\
	\includegraphics[trim={10cm 2cm 10cm 2cm}, clip = true,width=1.2cm]{figs/view45.png} &  \hspace{-0.5cm}
	\includegraphics[trim={10cm 2cm 10cm 2cm}, clip = true,width=1.2cm]{figs/view90.png}\\
	$ v_{\pi/4} $ & \hspace{-0.5cm} $ v_{\pi/2} $ \\
	\end{tabular}
	
	\vspace{1mm}
	\caption{Order of Rotational Symmetry}
	\label{fig:rot_sym}
\end{figure}
\fi
%		\includegraphics[trim={0 0 0 0}, clip = true,width=5.8cm]{figs/rot_sym3.jpg}
%		\put(-10,60){\Large $ \bX $}
%		\put(-102,155){\Large $ \bY $}
%		\put(-33, 128){\LARGE $ v $}
%		\put(-160, 10){\LARGE $ v' $}
%		\put(-50, 90){\Large $ \theta $} \\
%		{\large 3D Model} & {\large $  \mathcal{O} (\bY) = 2 $} & {\large $  \mathcal{O} (\bZ) = \infty $ }


%\vspace{-3mm}
\paragraph{Equivalent Viewpoint Sets} %For the axis, $ \bY $ in~\figref{fig:rot_sym} (middle), we have $ \mathcal{O}_{x} (\theta) = 2 $. 
Let us define the set of all pairs of equivalent viewpoints as $ E_o ( \bY ) = \{ (i, j) | v_j = \mathcal{R}_\theta ( \pi ) v_i \} $, with symmetry order $o \in \{ 2, 3, \infty \} $.  %Thus, we can similarly define, $ E_o ( \theta ), \forall o \in \{ 2, 3, \infty \} $. 
Note that $ E_1 (\theta) $ is a null set (object is asymmetric). In our case, we have $ E_2 (\theta)\subset E_4(\theta) \subset E_\infty (\theta) $ and $ E_3(\theta) \subset E_\infty (\theta) $.


%\subsection{Geometrical Constraints on Orders of Rotational Symmetry about Multiple Axes}
%\vspace{-3mm}
\paragraph{Geometric Constraints} We note that the orders of symmetries across multiple axes are not independent. We derive the following claim
\footnote{{\color{magenta} The proof of this claim is given in the supplementary material, available at \url{www.cs.utoronto.ca/~ecorona/supplementary_rotationalsymm.pdf}} }
 
%We use the following claim to constrain the output space of the predicted rotational symmetry in our approach. 

\begin{claim}
	\label{clm:order_constraint}
	If an object is not a sphere, then the following conditions must hold:
	\begin{enumerate}[noitemsep,label=(\alph*)]
		\item The object can have up to one axis with infinite order rotational symmetry.
		\item If an axis $ \theta $ has infinite order rotational symmetry, then the order of symmetry of any axis not orthogonal to $ \theta $ can only be one.%, \ie, other non-orthogonal axes can't have symmetric viewpoints. ({\color{red} re-phrase})
		\item If an axis $ \theta $ has infinite order rotational symmetry, then the order of symmetry of any axis orthogonal to $ \theta $ can be a maximum of two.
	\end{enumerate}
\end{claim}

Since in our experiments, none of the objects is a perfect sphere, we will use these constraints in Subsec.~\ref{sec:nw_arch} in order to improve the accuracy of our symmetry predicting network. 

%Since none of the objects in our dataset is a sphere, we use this to constrain the output space of our order predictions, \ie, order prediction of multiple axes is not an independent problem. In the next section we show how we incorporate these constraints for order prediction. The proof of this claim is given in the supplementary material.

